Higgs pair production via gluon fusion in the Two-Higgs-Doublet Model

We study the production of Higgs boson pairs via gluon fusion at the LHC in the Two-Higgs-Doublet Model. We present predictions at NLO accuracy in QCD, matched to parton showers through the MC@NLO method. A dedicated reweighting technique is used to improve the NLO calculation upon the infinite top-mass limit. We perform our calculation within the MadGraph5_aMC@NLO framework, along with the 2HDM implementation based on the NLOCT package. The inclusion of the NLO corrections leads to large K-factors and significantly reduced theoretical uncertainties. We examine the seven 2HDM Higgs pair combinations using a number of representative 2HDM scenarios. We show how the model-specific features modify the Higgs pair total rates and distribution shapes, leading to trademark signatures of an extended Higgs sector.

==> declare.tex <==

\newcommand{\lhcfits}{}
\newcommand{\feynhiggs}{}
\newcommand{\massboundsneutral}{CMS-PAS-HIG-13-002,CMS-PAS-HIG-13-021,CMS-PAS-HIG-13-014,CMS-PAS-HIG-13-025,Mankel:2014gwa}
\newcommand{\massboundscharged}{Aad:2012tj,Chatrchyan:2012vca,ATLAS-CONF-2013-090,Abbiendi:2013hk}

\newcommand{\unitarity}{Akeroyd:2000wc,Kanemura:1993hm,Maalampi:1991fb,Ginzburg:2005dt,Osland:2008aw}
\newcommand{\flavor}{Aubert:2007my,Su:2009fz,Aoki:2009ha,Mahmoudi:2012ej}
\newcommand{\vacuum}{Gunion:2002zf,Kanemura:1999xf,Ferreira:2009jb,Kastening:1992by,Velhinho:1994np,Nie:1998yn,Ferreira:2004yd,Maniatis:2006fs,Ferreira:2009jb}
\newcommand{\ewpo}{Toussaint:1978zm,Frere:1982ma,Bertolini:1985ia,Hollik:1986gg,Hollik:1987fg,Froggatt:1991qw,Grimus:2007if,Grimus:2008nb,He:2001tp}
\newcommand{\fits}{Ferreira:2011aa,Ferreira:2012my,Azatov:2012wq,Alves:2012ez,Cheon:2012rh,Bai:2012ex,Chiang:2013ixa,Grinstein:2013npa,Krawczyk:2013gia,Barroso:2013zxa,Coleppa:2013dya,Chen:2013rba,Chen:2013kt,Belanger:2013xza,Celis:2013rcs,Altmannshofer:2012ar,Craig:2013hca,Barger:2013ofa,Celis:2013ixa}
\newcommand{\collider}{Aoki:2011wd,Chang:2011kr,Arhrib:2011wc,Kanemura:2011kx,Mader:2012pm,Tsumura:2013yba,Harlander:2013mla}
\newcommand{\superiso}{Mahmoudi:2007vz,Mahmoudi:2008tp}
\newcommand{\higgsbounds}{Bechtle:2008jh,Bechtle:2011sb}

